Finite Time Regret Bounds for Minimum Variance Control of Autoregressive Systems with Exogenous Inputs

Minimum variance controllers have been employed in a wide-range of industrial applications. A key challenge experienced by many adaptive controllers is their poor empirical performance in the initial stages of learning. In this paper, we address the problem of initializing them so that they provide acceptable transients, and also provide an accompanying finite-time regret analysis, for adaptive minimum variance control of an auto-regressive system with exogenous inputs (ARX). Following [3], we consider a modified version of the Certainty Equivalence (CE) adaptive controller, which we call PIECE, that utilizes probing inputs for exploration. We show that it has a $C \log T$ bound on the regret after $T$ time-steps for bounded noise, and $C\log^2 T$ in the case of sub-Gaussian noise. The simulation results demonstrate the advantage of PIECE over the algorithm proposed in [3] as well as the standard Certainty Equivalence controller especially in the initial learning phase. To the best of our knowledge, this is the first work that provides finite-time regret bounds for an adaptive minimum variance controller.

==> appendices/lai_am.tex <==
from 2.15 of \cite{lai1986asymptotically}

==> appendices/notation.tex <==
\section{Notation}
$\mbf{0}$ is a vector consisting of all zeros.~If $M$ is a matrix, we let $\det(M)$ denote its determinant and $\Tr(M)$ denote its trace. For a vector $x$, we let $x'$ be its transpose.~If $x$ and $y$ are two vectors, we let $x\cdot y$ or $x'y$ denote their dot product. 



==> appendices/rho_dep.tex <==
\section{Regret Dependence upon $\rho$}\label{sec:rho_dep}
Note that
$$
\tau\ust_2 = \max\left\{\Bigg\lceil\frac{\log \br{\frac{B_u}{C_1 \|Y_0\|} }}{\log \rho} \Bigg\rceil ,0  \right\} \lesssim \log\br{1\slash \rho} .
$$

Also, $\tau\ust_3$ is the smallest value of $n$ that satisfies,
\al{
\left[ B_2 \times \frac{\log n}{\sqrt{n}} +  \sqrt{\frac{\log n}{n}} \right] \times \left[b_1\br{p+ 1 + \frac{C_1}{1-\rho}  \left\{1  +  \sum_{\ell=1}^{q} |b_\ell|   \right\} }\right] \le \frac{\delta^2_1}{2}.
}
Thus, 
$$
\tau\ust_3 \lesssim \br{\frac{1}{1-\rho}}^2.
$$
Also, $t\ust_4 \lesssim \frac{1}{\log \rho}$.


==> appendices/state_bound.tex <==
\section{Bounding $\|y(t)\|$}\label{sec:bound_state}
\subsubsection{Lemma 5-(ii) of~\cite{lai1987asymptotically}} 
We begin by stating this result. Suppose there exists a $K>0$ such that for sufficiently large $t$ we have,
\al{
|u(t)| \le \min \left\{ K|y(t)| , C \right\}.\label{cond:1}
}
Moreover, whenever $t\notin \cI$ and $K|y(t)|< C$, we have
\al{
|y(t+1) - w(t)| \ll C.\label{cond:2}
}
Then we have,
\al{
|y(t)| \ll C,~\mbox{ for sufficiently large } t.
}
\proof Note that we have
\al{
|u(t)| \le C,~w(t) \le C_1.
}
Hence, for sufficiently large $i$, and time $n_{i+1} > t> n_i + m_i$ if $K|y(t)|< C$, then from~\eqref{cond:2} we have,
\al{
|y(t+1)| &\le |w(t)| + \delta^2 C \notag\\
& \le C_1 + \delta^2 C\notag \\
& \le 2\delta^2 C. \qquad (C_1 \ll C)
}
We will use induction to prove that when $i$ is sufficiently large, then the following holds for times $t$ satisfying $n_i + \frac{m_i}{3} <t < n_{i+1}$,
\al{
|u(t)| < \delta C, ~ |y(t+1)| < \delta^2 C.\label{eq:tpt}
}
~\eqref{eq:tpt} has already been shown for $n_i + \frac{m_i}{3} < t<n_i + m_i$ in Lemma 5-(i), (note that $|u(t)|\le C_1$ was assumed since the very beginning for $t\in\cI$). Next, consider time $s$ satisfying $n_{i+1} > s>n_i + m_i$, and assume that~\eqref{eq:tpt} holds for $n_i + \frac{m_i}{3} \le t\le s$. We will show that~\eqref{eq:tpt} also holds for time $t=s+1$. Consider,
\al{
K |y(s+1)| &\le K \delta^2 C \qquad (\mbox{ induction hypothesis }~\eqref{eq:tpt}) \\
& < C  \qquad (\mbox{ choose } \delta < \frac{1}{\sqrt{K}}),
}
which shows that the conditions for~\eqref{cond:2} are satisfied. Hence,~\eqref{cond:2} yields us
\al{
|y(s+2)| \le \delta^2 C.
}
It thus remains to show $|u(s+1)|< \delta \cdot C$. We have,
\al{
|u(s+1)| &\le K|y(s+1)| \qquad  (\mbox{from} ~~\eqref{cond:1})\notag\\
&\le K \delta^2 \cdot C \qquad (\mbox{ induction hypothesis }~\eqref{eq:tpt})  \notag\\
&\le \delta \cdot C (\mbox{ choose }\delta < \frac{1}{K}). 
}
This completes the induction, and hence proves that~\eqref{eq:tpt} holds.  

Thus, we have shown that for times $t\notin \cI$, we have $|u(t)|\ll C$. Also, $|u(t)|\ll C$ also holds for $t\in\cI$ by design~\eqref{ineq:bd1}. Hence, we have shown that 
\al{
|u(t)|\ll C,~\forall t.\label{ineq:u}
}
From~\eqref{ineq:bd2} we already have
\al{
|w(t)| \ll C,~ \forall t.\label{ineq:w}
}
Upon substituting~\eqref{ineq:u},~\eqref{ineq:w} into~\eqref{ineq:1}, we obtain the following,
\al{
|y(t)| \ll C~\forall t.\label{ineq:y}
}

\qed 


==> files/introduction_AM.tex <==
\section{Introduction}

Adaptive control theory focuses on developing efficient controllers when the system model is unknown.
Due to extensive industrial applications, adaptive control of linear systems is arguably 
the most exhaustively studied problem in control theory.  Traditionally, the analysis of adaptive controllers has focused on the asymptotic properties \cite{lai1982asymptotic,lai1986asymptotically,lai1987asymptotically}. With the advent of reinforcement learning, there has been a renewed focus on the topic of adaptive control of linear systems in recent years \cite{simchowitz2020naive,dean2019safely}. 
Although these recent works consider the same problem as traditional adaptive control literature, they focus on the finite-time analysis and sample complexity of such adaptive controllers instead of only asymptotic properties.

The recent works on adaptive linear systems have majorly focused on the popular LQG problem. In this paper, we revisit another popular control problem called the minimum variance controller.

Consider a simple linear system given by: 
$y_{t+1}=ay_t+bu_t+w_{t+1}$. Then the minimum variance controller wants to minimize the expected variance of the output $y_t$. The development of the minimum variance controller can be tracked back to the paper-making industry wanting to produce papers of a consistent width.  This has wide-range of industrial applications \cite{astrom1987adaptive,dumont1982self,seborg1986adaptive,sastry1977self,bongtsson1984experiences,kallstrom1979adaptive}. 

If the system parameter $a,b$ were known then the optimal control law is given by $u_t=-\frac{a}{b}y_t$.  In case, the parameters are not known, the adaptive minimum variance controller should choose the control input $u_t$  in such a way that it efficiently estimates the system parameter $a,b$ while keeping the variance $(y_t-w_t)$ low. This trade-off is popularly known as the dual control problem \cite{}, or exploration vs. exploitation dilemma in reinforcement learning.

One of the initial approaches to this resolve this dilemma is the well-known "self-tuning regulator" approach proposed in \cite{aastrom1973self}.
Based on the ''separation principle'', i.e. one computes the optimal controller assuming the true system was known i.e., $u_t=\frac{-a}{b}y_t$, and then replaces the parameters by the least-squared estimates: $u_t=\frac{-\hat{a}_t}{\hat{b}_t}y_t,\text{ where } \hat{a}, \hat{b}$ are least-squared estimates of $(a,b)$. This is also called the Certainty Equivalence (CE) rule.
A similar approach was proposed in econometrics 
\cite{anderson1976some} for an even simpler model $y_{t+1}=a+bu_t+w_{t+1}$. They proposed the following control law:  $u_t = k_l \vee \frac{\hat{a}_t}{\hat{b}_t}\wedge k_u\footnote{where $\vee,\wedge$ denote maximum and minimum respectively.}$, where, $k_l,k_u$ are lower and upper bounds respectively on the ratio $\frac{a}{b}$ that are assumed to be known apriori. It was shown that such the estimates $\frac{\hat{a}_t}{\hat{b}_t}$  controllers do not converge to  $\frac{a}{b}$ with a positive probability~\cite{lai1982iterated}.

This issue was resolved in \cite{lai1986asymptotically,lai1987asymptotically} by proposing a modification to the Certainty Equivalence approach. They introduce ``exploration episodes''. For times within such episodes, the algorithm utilizes ``probing inputs'' which ensures that the estimates $(\hat{a}_t,\hat{b}_t)$ are asymptotically consistent. They also introduced the notion of "regret" for a minimum variance control problem, which quantifies the sub-optimality incurred in the variance of $y_t$ while estimating the parameters $(a,b)$. The regret is defined as $\cR_T=\sum_{t=1}^T(y_t-w_t)^2$. They showed that the Certainty Equivalence with "exploration episode" achieves asymptotic logarithmic regret. More specifically, \cite{lai1987asymptotically} showed that for an ARX system: 
\nal{
y_t= a_1 y_{t-1} + a_2 y_{t-2} + \ldots +a_p y_{t-p} +b_1 u_{t-1} + b_2 u_{t-2}+\cdots + b_q u_{t-q}+ w_t, ~ \forall~ t \in \bN 
,}
the asymptotic regret is as given by:
\nal{\limsup_{T \to \infty} \frac{R_T}{\log T}\le \sigma^2(p+q-1).}

As mentioned earlier, recently we have seen a great interest in finite time analysis of adaptive controllers in the reinforcement learning literature. Surprisingly, the finite time analysis of learning algorithms for a minimum variance controller has been an open problem until now. In this paper, we take the first step in that direction and provide the first finite time regret bounds for an adaptive minimum variance controller.

\subsection{LQG Controllers vs Minimum Variance Controllers}
Another widely popular adaptive control problem is when the controller's cost at time $t$ is quadratic in both output and control input. i.e., for a  linear system, $Y_{t+1}=AY_t+BU_t+W_{t+1}$, the cost at time $t$ is  $ Y_t^{\intercal}QY_t + U^{\intercal}_t RU_t$, where $Q$ is a positive semi-definite matrix 
 and $R$ is positive definite matrix. 
This problem is popularly known as the LQG control problem. When the system matrices $A, B$ are known the optimal control is given by $U_t=K(A, B)Y_t$, where $K(A, B)$ is obtained by solving a discrete algebraic Riccati equation.

The recent works on the finite-time analysis of linear systems have been almost exclusively focused on the LQG setting. A wide-range of adaptive controllers like OFU \cite{abbasi2011regret}, TS \cite{abeille_17}, CEC \cite{simchowitz2020naive,jedra2022minimal}, RBMLE \cite{mete2022augmented} have been shown to achieve $C\sqrt{T}$ finite time regret. Notably, \cite{simchowitz2020naive} showed that a simple modification of the Certainty Equivalence controller achieves a $C\sqrt{T}$ regret with optimal pre-constant $C$.

One might wonder that the minimum variance controller seems to be a special case of the LQG controller with $Q=I$ and $R=0$. It is important to note that the solution of an optimal controller in the LQG setting requires $R$ to be a positive definite matrix and hence the minimum variance controller requires independent attention. 
Another important difference between the optimal average cost for a given system with parameters $(A, B)$ in the LQG setting depends on the system parameters $(A, B)$. Meanwhile, the optimal average cost in minimum variance is only dependent on the variance of the system noise irrespective of the system parameters. Due to this fact, optimistic learning algorithms like OFU \cite{abbasi2011regret} and RBMLE \cite{mete2022augmented} can not be adapted for minimum variance controllers.
\am{I am trying to highlight the need to seperately studying the adaptive minimum variance control problem in this paragraph.}
\subsection{Our Contributions}
In this work, we consider the problem of learning to 
provide the finite-time regret analysis of an ARX system.
Inspired by \cite{lai1986asymptotically,lai1987asymptotically}We consider a modified version of the Certainty Equivalence controller which incorporates probing inputs for exploration, which we call PIECE. Our main theoretical contribution is an upper bound on the regret of the PIECE algorithm. We provide regret bounds for two separate scenarios: 
\begin{itemize}
    \item Bounded Noise: If the system noise $w_t$ is bounded, we show that the regret is $C\log T$.
    \item Unbounded Noise: If the system noise $w_t$ is sub-Gaussian, we show that the regret of the PIECE algorithm is $C\log^2 T$.
\end{itemize}
We show that a logarithmic regret is achievable in the minimum variance control setting, unlike the LQG setting. We also provide simulation results for various ARX systems to validate our theoretical results. Comparing the performance of the PIECE algorithm with that of the standard Certainty Equivalence controller, our simulation results establish the advantage of PIECE over Certainty Equivalence.
  
\subsection{Organization of the Paper}
We describe the ARX system model and notations in Section \ref{sec:system_model}. In Section \ref{sec:algo}, we describe an adaptive minimum variance control algorithm called PIECE. Our main technical results on regret analysis are provided in Section \ref{sec:regret}. Section \ref{sec:simulations} includes the results of our simulation experiments for various ARX systems. We conclude with a brief discussion on the open problems in Section \ref{sec:discussion}. All the proofs and details on experiments are provided in the appendices.



 


